Social Fraud Detection Review: Methods, Challenges and Analysis

Social reviews have dominated the web and become a plausible source of product information. People and businesses use such information for decision-making. Businesses also make use of social information to spread fake information using a single user, groups of users, or a bot trained to generate fraudulent content. Many studies proposed approaches based on user behaviors and review text to address the challenges of fraud detection. To provide an exhaustive literature review, social fraud detection is reviewed using a framework that considers three key components: the review itself, the user who carries out the review, and the item being reviewed. As features are extracted for the component representation, a feature-wise review is provided based on behavioral, text-based features and their combination. With this framework, a comprehensive overview of approaches is presented including supervised, semi-supervised, and unsupervised learning. The supervised approaches for fraud detection are introduced and categorized into two sub-categories; classical, and deep learning. The lack of labeled datasets is explained and potential solutions are suggested. To help new researchers in the area develop a better understanding, a topic analysis and an overview of future directions is provided in each step of the proposed systematic framework.

==> tikzlibrarytimeline.code.tex <==
% * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *
% COPYRIGHT 2014 - Claudio Fiandrino
% Released under the LaTeX Project Public License v1.3c or later
% 
% email: <claudio dot fiandrino at gmail dot com>
%
% Timeline TikZ library version 0.3b - 25/02/2019

\usetikzlibrary{backgrounds,calc}

\pgfkeys{/tikz/.cd,
  timespan/.store in=\timespan,
  timespan=,
  timeline width/.store in=\timelinewidth,
  timeline width=30,
  timeline height/.store in=\timelineheight,
  timeline height=1,
  timeline offset/.store in=\timelineoffset,
  timeline offset=0.15,
  initial week/.store in=\initialweek,
  initial week=1,
  end week/.store in=\endweek,
  end week=2,
  time point/.store in=\timepoint,
  time point=0.5,
  between day/.style args={#1 and #2 in #3}{% auxiliary style for days
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between week/.style args={#1 and #2 in #3}{% style for weeks
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between month/.style args={#1 and #2 in #3}{% auxiliary style for months
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between year/.style args={#1 and #2 in #3}{% auxiliary style for years
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  involvement degree/.store in=\involvdegree,
  involvement degree=2cm,
  phase color/.store in=\phasecol,
  phase color=red!50!orange,
  phase appearance/.style={
    circle,
    opacity=0.3,
    minimum size=\involvdegree,
    fill=\phasecol
  },
}
% settings to customize aspect of timeline
\newif\ifcustominterval
\pgfkeys{/tikz/timeline/.cd,
  custom interval/.is if=custominterval,
  custom interval=false,
}

% settings to deploy milestones
\pgfkeys{/tikz/milestone/.cd,
  at/.store in=\msstartpoint,
  at=phase-1.north,
  circle radius/.store in=\milestonecircleradius,
  circle radius=0.1cm,
  direction/.store in=\msdirection,
  direction=90:2cm,
  text/.store in=\mstext,
  text={},
  text options/.code={\tikzset{#1}},
}

\newcommand{\reftimespan}{\MakeLowerCase{\timespan}}

\newcommand{\timeline}[2][]{
  \pgfkeys{/tikz/timeline/.cd,#1}
  \draw[fill,opacity=0.8] (0,0) rectangle (\timelinewidth,\timelineheight);
  \shade[top color=black, bottom color=white,middle color=black!20]
    (0,0) rectangle (\timelinewidth,-\timelineoffset);
  \shade[top color=white, bottom color=black,middle color=black!20]  
    (0,\timelineheight) rectangle (\timelinewidth,\timelineheight+\timelineoffset);

  \ifcustominterval%
    \foreach \smitem [count=\tlmxi] in {#2}  {\global\let\maxsmitem\tlmxi}%
  \else%
    \foreach \smitem [count=\tlmxi] in {1,...,#2}  {\global\let\maxsmitem\tlmxi}%
  \fi%
  
  \pgfmathsetmacro\position{\timelinewidth/(\maxsmitem+1)}
  \node at (0,0.5\timelineheight)(\timespan-0){\phantom{Week 0}};
 
  \ifcustominterval%
    \foreach \x[count=\tlmxi] in {#2}{%
      \node[text=white,text depth=0pt]at +(\tlmxi*\position,0.5\timelineheight) (\timespan-\tlmxi) {\timespan\ \x};%
    }%
  \else%
    \foreach \x[count=\tlmxi] in {1,...,#2}{%
      \node[text=white, text depth=0pt]at +(\tlmxi*\position,0.5\timelineheight) (\timespan-\tlmxi) {\timespan\ \x};%
    }%
  \fi%  
}

\newcounter{involv}
\setcounter{involv}{0}

\newcommand{\phase}[1]{
\stepcounter{involv}
\node[phase appearance,#1] 
 (phase-\theinvolv)
 at ($(\timespan-\initialweek)!\timepoint!(\timespan-\endweek)$){};
}

\newcommand{\initialphase}[1]{
\node[phase appearance,#1,anchor=west,between week=0 and 1 in 0,] 
 (phase-\theinvolv)
 at ($(\timespan-0)!0!(\timespan-1)$){};
\setcounter{involv}{0} 
}

\newenvironment{phases}{\begin{pgfonlayer}{background}}{\end{pgfonlayer}}

\newcommand{\addmilestone}[1]{
\pgfkeys{/tikz/milestone/.cd,#1}
\draw[double,fill] (\msstartpoint) circle [radius=\milestonecircleradius];
\draw(\msstartpoint)--++(\msdirection)node[/tikz/milestone/text options]{\mstext};
}

% HISTORY
% 0.1 -> initial release
% 0.2 -> customizable timespan label
% 0.3 -> \timeline command with custom intervals
%             styles ``between x''
%             removed unnecessary call to xstring
% 0.3a -> text depth for timeline labels
% 0.3b -> \xi conflict - thanks Enrico Gregorio (egreg) https://tex.stackexchange.com/q/476089
